Position Masking for Improved Layout-Aware Document Understanding

Natural language processing for document scans and PDFs has the potential to enormously improve the efficiency of business processes. Layout-aware word embeddings such as LayoutLM have shown promise for classification of and information extraction from such documents. This paper proposes a new pre-training task called that can improve performance of layout-aware word embeddings that incorporate 2-D position embeddings. We compare models pre-trained with only language masking against models pre-trained with both language masking and position masking, and we find that position masking improves performance by over 5% on a form understanding task.

==> extras.tex <==
% \section*{Acknowledgments}
% The acknowledgments should go immediately before the references. Do not number the acknowledgments section.
% \textbf{Do not include this section when submitting your paper for review.}
\pagebreak 
\section*{Ethical Considerations}
% \cfd{See \url{https://2021.naacl.org/ethics/faq/\#should-i-have-an-ethical-considerations-section-in-my-paper} and  \url{https://2021.naacl.org/ethics/review-questions/}
% Note that we can write up to a page in this section; it doesn't count towards the 4-page limit}
\subsection*{Data}
We use existing datasets with the exception of a supplemental portion of our pre-training data.
In collecting this portion, we have attempted to follow ethical standards in the following ways:
\begin{itemize}
    \item We believe our dataset collection respects intellectual property by being ``fair use.'' We have collected a relatively small fraction of the overall tobacco litigation documents (180,000 pages out of a total of over 92 million pages\footnote{\url{https://www.industrydocuments.ucsf.edu/tobacco/about/overview/}}). The purpose and character of the use is for research. The nature of the use does not affect the potential market for or value of any of pages that might be copyrighted. We balance reproducibility with intellectual property by making public which document pages we used, rather than posting copies of the documents themselves.
    \item The dataset is in English. There is no reason to believe the technology could not work on other high-resource languages if similar datasets were collected.
    \item Because the dataset is used for pre-training, noisy data is preferable over manually curated data, as it is more realistic.
    \item The source we collected from, UCSF Industry Documents Library, redacts private information from the documents.\footnote{\url{https://www.industrydocuments.ucsf.edu/help/privacy/}}
\end{itemize}

\subsection*{Technology}
The technology our contribution facilitates is automated processing of business documents and other document scans.
It is intended to help organizations dealing with overwhelming numbers of documents to route them appropriately based on their type and to extract information from them.
The only risk we have identified is the potential replacement of human labor with automation, which is inherent in any labor-saving technology.
Moreover, given the high accuracy demanded by enterprises for this type of task, the technology is more likely to be used as a tool to make workers' jobs easier, rather than supplanting workers entirely, for the foreseeable future.

\subsection*{Environmental Impact}
We have attempted to limit the environmental impact of our experiments by reducing their size.
Rather than pre-training on 11 million pages, we selected the smallest pre-training size reported in LayoutLM, 500,000 pages.
We pre-trained all models for 6 epochs. 
Using 8 V100 GPUs, pre-training a model took approximately 4.5 hours. 

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
